Milky Way Cepheid Standards for Measuring Cosmic Distances and Application to Gaia DR2: Implications for the Hubble Constant

We present HST photometry of a selected sample of 50 long-period, low-extinction Milky Way Cepheids measured on the same WFC3 F555W, F814W, and F160W-band photometric system as extragalactic Cepheids in SN Ia hosts. These bright Cepheids were observed with the WFC3 spatial scanning mode in the optical and near-infrared to mitigate saturation and reduce pixel-to-pixel calibration errors to reach a mean photometric error of 5 millimags per observation. We use the new Gaia DR2 parallaxes and HST photometry to simultaneously constrain the cosmic distance scale and to measure the DR2 parallax zeropoint offset appropriate for Cepheids. We find a value for the zeropoint offset of -46 +/- 13 muas or +/- 6 muas for a fixed distance scale, higher than found from quasars, as expected, for these brighter and redder sources. The precision of the distance scale from DR2 has been reduced by a factor of 2.5 due to the need to independently determine the parallax offset. The best fit distance scale is 1.006 +/- 0.033, relative to the scale from Riess et al 2016 with H0=73.24 km/s/Mpc used to predict the parallaxes photometrically, and is inconsistent with the scale needed to match the Planck 2016 CMB data combined with LCDM at the 2.9 sigma confidence level (99.6%). At 96.5% confidence we find that the formal DR2 errors may be underestimated as indicated. We identify additional error associated with the use of augmented Cepheid samples utilizing ground-based photometry and discuss their likely origins. Including the DR2 parallaxes with all prior distance ladder data raises the current tension between the late and early Universe route to the Hubble constant to 3.8 sigma (99.99 %). With the final expected precision from Gaia, the sample of 50 Cepheids with HST photometry will limit to 0.5% the contribution of the first rung of the distance ladder to the uncertainty in the Hubble constant.

==> bigtable2.tex <==
\startlongtable
\begin{deluxetable*}{ccccccccccccccc}
\tabletypesize{\scriptsize}
\tablewidth{0pt}
\tablenum{1}
\tablecaption{Photometric Data for MW Cepheids\label{tb:phot}}
\tablehead{\colhead{Cepheid} &  \colhead{log Period} & \colhead{$F555W$} & \colhead{$\sigma$}  & \colhead{$n$} & \colhead{$F814W$} & \colhead{$\sigma$}  & \colhead{$n$} & \colhead{$F160W^a$} & \colhead{$\sigma$}  & \colhead{$n$} & \colhead{$m^{W,b}_H$} & \colhead{$\sigma$}  & \colhead{$\pi_{R16}^{c}$} & \colhead{$\sigma$} \\
\colhead{} & \colhead{} & \colhead{(mag)} &  \colhead{} & \colhead{(epochs)} &  \colhead{(mag)} &  \colhead{} & \colhead{(epochs)} & \colhead{(mag)} &  \colhead{} & \colhead{(epochs)} &  \colhead{(mag)} &  \colhead{}  &  \colhead{(mas)}    &  \colhead{}}
\startdata
AA-GEM &  1.053  &  9.9130  &  0.029  &  1  &  8.542  &  0.025  &      1  &  7.348  &  0.017  &      1  &  6.871  &  0.023   &  0.254  &  0.005  \\
AD-PUP &  1.133  &  10.015  &  0.028  &  1  &  8.675  &  0.023  &      1  &  7.488  &  0.020  &      1  &  7.023  &  0.024   &  0.210  &  0.005  \\
AQ-CAR &  0.990  &  8.9836  &  0.020  &  2  &  7.854  &  0.009  &      2  &  6.766  &  0.007  &      3  &  6.382  &  0.011   &  0.350  &  0.007  \\
AQ-PUP &  1.479  &  8.8671  &  0.018  &  2  &  7.120  &  0.014  &      2  &  5.487  &  0.013  &      4  &  4.864  &  0.016   &  0.338  &  0.007  \\
BK-AUR &  0.903  &  9.5609  &  0.036  &  1  &  8.220  &  0.038  &      1  &  7.015  &  0.021  &      1  &  6.549  &  0.029   &  0.369  &  0.008  \\
BN-PUP &  1.136  &  10.051  &  0.033  &  1  &  8.505  &  0.017  &      1  &  7.198  &  0.015  &      1  &  6.653  &  0.021   &  0.248  &  0.005  \\
CD-CYG &  1.232  &  9.1207  &  0.011  &  3  &  7.468  &  0.012  &      3  &  5.900  &  0.012  &      5  &  5.314  &  0.014   &  0.398  &  0.008  \\
CP-CEP &  1.252  &  10.757  &  0.015  &  1  &  8.638  &  0.052  &      1  &  6.871  &  0.022  &      1  &  6.105  &  0.030   &  0.268  &  0.006  \\
CR-CAR &  0.989  &  11.750  &  0.019  &  1  &  9.973  &  0.018  &      1  &  8.384  &  0.014  &      1  &  7.750  &  0.017   &  0.187  &  0.004  \\
CY-AUR &  1.141  &  12.052  &  0.012  &  1  &  9.953  &  0.020  &      1  &  8.106  &  0.025  &      1  &  7.348  &  0.027   &  0.179  &  0.004  \\
DD-CAS &  0.992  &  10.036  &  0.007  &  3  &  8.523  &  0.011  &      3  &  7.108  &  0.012  &      4  &  6.576  &  0.013   &  0.319  &  0.006  \\
DL-CAS &  0.903  &  9.1059  &  0.019  &  1  &  7.569  &  0.022  &      1  &  6.238  &  0.018  &      1  &  5.697  &  0.021   &  0.547  &  0.011  \\
DR-VEL &  1.049  &  9.7083  &  0.034  &  1  &  7.770  &  0.020  &      1  &  6.183  &  0.021  &      1  &  5.487  &  0.026   &  0.484  &  0.011  \\
GQ-ORI &  0.935  &  8.7199  &  0.020  &  1  &  7.632  &  0.024  &      1  &  6.523  &  0.032  &      1  &  6.155  &  0.034   &  0.422  &  0.010  \\
HW-CAR &  0.964  &  9.2782  &  0.016  &  2  &  8.007  &  0.013  &      2  &  6.798  &  0.005  &      3  &  6.359  &  0.009   &  0.368  &  0.007  \\
KK-CEN &  1.086  &  11.598  &  0.017  &  1  &  9.862  &  0.021  &      1  &  8.292  &  0.015  &      1  &  7.674  &  0.018   &  0.167  &  0.003  \\
KN-CEN &  1.532  &  10.062  &  0.023  &  2  &  7.924  &  0.017  &      2  &  5.856  &  0.006  &      5  &  5.083  &  0.013   &  0.282  &  0.005  \\
RW-CAM$^*$ &  1.215  &  8.8673  &  0.015  &  1  &  7.044  &  0.014  &      1  &  5.451  &  0.021  &      1  &  4.799  &  0.022   &  0.517  &  0.011  \\
RW-CAS &  1.170  &  9.3719  &  0.021  &  1  &  7.863  &  0.016  &      1  &  6.483  &  0.022  &      1  &  5.952  &  0.024   &  0.326  &  0.007  \\
RY-CAS &  1.084  &  10.075  &  0.019  &  1  &  8.333  &  0.040  &      1  &  6.715  &  0.010  &      1  &  6.094  &  0.020   &  0.347  &  0.007  \\
RY-SCO &  1.308  &  8.2067  &  0.012  &  3  &  6.206  &  0.010  &      3  &  4.408  &  0.010  &      3  &  3.688  &  0.012   &  0.751  &  0.014  \\
RY-VEL$^*$ &  1.449  &  8.5234  &  0.036  &  1  &  6.757  &  0.016  &      1  &  5.211  &  0.017  &      1  &  4.581  &  0.023   &  0.403  &  0.009  \\
S-NOR &  0.989  &  6.5779  &  0.011  &  1  &  5.410  &  0.012  &      1  &  4.391  &  0.012  &      1  &  3.992  &  0.014   &  1.053  &  0.021  \\
S-VUL &  1.839  &  9.1668  &  0.008  &  3  &  6.862  &  0.012  &      3  &  4.885  &  0.010  &      4  &  4.047  &  0.011   &  0.287  &  0.006  \\
SS-CMA &  1.092  &  10.121  &  0.012  &  4  &  8.444  &  0.008  &      4  &  6.894  &  0.011  &      3  &  6.299  &  0.012   &  0.312  &  0.006  \\
SV-PER$^*$ &  1.046  &  9.2186  &  0.016  &  1  &  7.760  &  0.014  &      1  &  6.435  &  0.027  &      1  &  5.924  &  0.028   &  0.397  &  0.009  \\
SV-VEL &  1.149  &  8.7316  &  0.026  &  1  &  7.302  &  0.009  &      1  &  6.024  &  0.010  &      1  &  5.524  &  0.015   &  0.409  &  0.008  \\
SV-VUL &  1.653  &  7.2675  &  0.047  &  1  &  5.648  &  0.033  &      1  &  4.214  &  0.027  &      1  &  3.641  &  0.035   &  0.457  &  0.011  \\
SY-NOR &  1.102  &  9.8284  &  0.023  &  1  &  7.925  &  0.038  &      1  &  6.214  &  0.013  &      1  &  5.531  &  0.022   &  0.438  &  0.009  \\
SZ-CYG &  1.179  &  9.6209  &  0.013  &  2  &  7.756  &  0.017  &      2  &  6.004  &  0.008  &      3  &  5.336  &  0.012   &  0.427  &  0.008  \\
T-MON$^*$ &  1.432  &  6.0680  &  0.023  &  1  &  4.828  &  0.016  &      1  &  3.725  &  0.021  &      1  &  3.298  &  0.024   &  0.746  &  0.016  \\
U-CAR &  1.589  &  6.3852  &  0.038  &  1  &  4.967  &  0.023  &      1  &  3.768  &  0.019  &      1  &  3.272  &  0.026   &  0.596  &  0.013  \\
UU-MUS &  1.066  &  9.9212  &  0.024  &  1  &  8.457  &  0.025  &      1  &  7.108  &  0.010  &      1  &  6.595  &  0.017   &  0.283  &  0.006  \\
V0339-CEN &  0.976  &  8.8402  &  0.024  &  1  &  7.321  &  0.016  &      1  &  5.990  &  0.024  &      1  &  5.455  &  0.026   &  0.548  &  0.012  \\
V0340-ARA &  1.318  &  10.460  &  0.024  &  1  &  8.554  &  0.014  &      1  &  6.808  &  0.012  &      1  &  6.124  &  0.016   &  0.241  &  0.005  \\
VW-CEN &  1.177  &  10.379  &  0.031  &  1  &  8.718  &  0.023  &      1  &  7.158  &  0.010  &      1  &  6.569  &  0.018   &  0.243  &  0.005  \\
VX-PER &  1.037  &  9.4589  &  0.008  &  4  &  7.906  &  0.006  &      3  &  6.470  &  0.009  &      5  &  5.922  &  0.010   &  0.403  &  0.008  \\
VY-CAR &  1.276  &  7.6162  &  0.014  &  5  &  6.253  &  0.007  &      4  &  4.991  &  0.004  &      6  &  4.517  &  0.007   &  0.538  &  0.010  \\
VZ-PUP &  1.365  &  9.7715  &  0.033  &  1  &  8.262  &  0.022  &      1  &  6.931  &  0.017  &      1  &  6.400  &  0.023   &  0.198  &  0.004  \\
WX-PUP &  0.951  &  9.1909  &  0.030  &  1  &  7.944  &  0.012  &      1  &  6.807  &  0.010  &      1  &  6.378  &  0.016   &  0.372  &  0.007  \\
WZ-SGR &  1.339  &  8.2021  &  0.012  &  6  &  6.481  &  0.013  &      6  &  4.858  &  0.009  &      4  &  4.245  &  0.011   &  0.554  &  0.011  \\
X-CYG &  1.214  &  6.5295  &  0.020  &  1  &  5.230  &  0.049  &      1  &  4.080  &  0.033  &      1  &  3.630  &  0.039   &  0.887  &  0.023  \\
X-PUP &  1.414  &  8.6949  &  0.019  &  3  &  7.128  &  0.010  &      3  &  5.628  &  0.008  &      4  &  5.075  &  0.012   &  0.338  &  0.006  \\
XX-CAR &  1.196  &  9.4627  &  0.027  &  1  &  8.067  &  0.015  &      1  &  6.833  &  0.022  &      1  &  6.346  &  0.025   &  0.261  &  0.006  \\
XY-CAR &  1.095  &  9.4660  &  0.011  &  4  &  7.927  &  0.009  &      3  &  6.455  &  0.006  &      6  &  5.913  &  0.008   &  0.371  &  0.007  \\
XZ-CAR &  1.221  &  8.7725  &  0.017  &  3  &  7.217  &  0.006  &      3  &  5.770  &  0.007  &      4  &  5.221  &  0.010   &  0.422  &  0.008  \\
YZ-CAR &  1.259  &  8.8644  &  0.016  &  3  &  7.401  &  0.007  &      3  &  5.991  &  0.013  &      5  &  5.478  &  0.015   &  0.354  &  0.007  \\
YZ-SGR &  0.980  &  7.4662  &  0.021  &  1  &  6.176  &  0.014  &      1  &  5.103  &  0.020  &      1  &  4.657  &  0.022   &  0.786  &  0.017  \\
Z-LAC &  1.037  &  8.5686  &  0.022  &  1  &  7.157  &  0.015  &      1  &  5.917  &  0.018  &      1  &  5.424  &  0.021   &  0.507  &  0.011  \\
Z-SCT &  1.111  &  9.7535  &  0.019  &  2  &  8.079  &  0.021  &      2  &  6.513  &  0.008  &      3  &  5.918  &  0.014   &  0.362  &  0.007  \\
\hline
\enddata
\tablecomments{$^a$Does not include addition of $0.052 \pm 0.014$ mag to correct CRNL 6.4 dex between MW and extragalactic Cepheids.}
\tablecomments{$^b$Includes addition of $0.052 \pm 0.014$ mag to correct CRNL 6.4 dex between MW and extragalactic Cepheids.}
\tablecomments{$^c$ $\pi_{R16}=10^{-0.2(\mu-10)}$ where $\mu=m^W_H-M^W_H$ and $M^W_H$ is the absolute Wesenheit magnitude determined from the Cepheid period and the distance scale from \cite{Riess:2016} where $H_0$=73.24 \kmsmpc as discussed in the text.}
\tablecomments{$^*$ Not used in final analysis, see text}
\end{deluxetable*}

